On the Optimal Sample Complexity for Best Arm Identification

We study the best arm identification (BEST-1-ARM) problem, which is defined as follows. We are given $n$ stochastic bandit arms. The $i$th arm has a reward distribution $D_i$ with an unknown mean $\mu_{i}$. Upon each play of the $i$th arm, we can get a reward, sampled i.i.d. from $D_i$. We would like to identify the arm with the largest mean with probability at least $1-\delta$, using as few samples as possible. We provide a nontrivial algorithm for BEST-1-ARM, which improves upon several prior upper bounds on the same problem. We also study an important special case where there are only two arms, which we call the sign problem. We provide a new lower bound of sign, simplifying and significantly extending a classical result by Farrell in 1964, with a completely new proof. Using the new lower bound for sign, we obtain the first lower bound for BEST-1-ARM that goes beyond the classic Mannor-Tsitsiklis lower bound, by an interesting reduction from Sign to BEST-1-ARM. We propose an interesting conjecture concerning the optimal sample complexity of BEST-1-ARM from the perspective of instance-wise optimality.

==> algo.tex <==
%!TEX root=bestarm.tex
\newcommand{\seqn}{\mathbb{S}}
\newcommand{\terround}{\kappa}

\section{Algorithm for \sign}
\label{sec:algorithm-sign}

In this section we prove Theorem~\ref{thm:FAST-ALGO} by presenting a class of 
algorithms for \sign. 
Each algorithm here is in fact a simple variant of the \EXPGAPELIMINATION\ algorithm in \cite{karnin2013almost}. 

Now, we begin our description of the algorithm.
Our algorithm takes an infinite sequence $\seqn=\{\refseq_i\}_{i=1}^{+\infty}$ as input, which we call
the {\em reference sequence}.

\begin{defi}
	We say an infinite sequence $\seqn=\{\refseq_i\}_{i=1}^{+\infty}$ is a {\em reference sequence} if 
	the following statements hold:    
	\begin{enumerate}
		\item $0<\refseq_i<1$, for all $i$.
		\item There exists a constant $0<c<1$ such that for all $i$, $\refseq_{i+1} \le c \cdot \refseq_{i}$.
	\end{enumerate}
\end{defi}

Our algorithm \TESTSIGN\ takes a confidence level $\delta$ and the reference 
sequence $\{ \refseq_i \}$ as input. It runs in rounds.
In the $r$th round, 
the algorithm takes a number of samples (the actual number depends on $r$, and can be found in 
Algorithm~\ref{algo:FAST-ALGO-SIGN}) from the arm and let $\widehat{\mu}^r$ be the empirical mean.
If $\widehat{\mu}^r\in \xi\pm \refseq_r/2$, we decide that the gap $\Delta$ is smaller than the reference gap $\refseq_r$
and we should proceed to the next round with a smaller reference gap.
If $\widehat{\mu}^r$ is larger than $\xi + \refseq_r/2$,
we decide $\mu>\xi$.
If $\widehat{\mu}^r$ is smaller than $\xi - \refseq_r/2$,
we decide $\mu<\xi$.
The pseudocode can be found in algorithm~\ref{algo:FAST-ALGO-SIGN}.

\begin{algorithm}[t]
\hrule\smallskip	
\LinesNumbered
\setcounter{AlgoLine}{0}
	\caption{\TESTSIGN($A,\delta,\{ \refseq_i \}$)}
	\label{algo:FAST-ALGO-SIGN}
\hrule\medskip
	\KwData{The single arm $A$ with unknown mean $\mu \ne \xi$, confidence level $\delta$, the reference 
		sequence $\{ \refseq_i \}$.}
	\KwResult{Whether $\mu > \xi$ or $\mu < \xi$.}
	\smallskip
	\For{r = 1 to $+\infty$}{
		$\epsilon_r = \refseq_r/2$
		
		$\delta_{r} = \delta/10r^2$
		
		Pull $A$ for $t_r = 2\ln(2/\delta_r)/\epsilon_r^2$ times. Let $\widehat{\mu}^{r}$ denote its average reward.
		
		\uIf{$\widehat{\mu}^r > \xi + \epsilon_r$}{
			{\bf Return} $\mu > \xi$
		}
		
		\uIf{$\widehat{\mu}^r < \xi - \epsilon_r$}{
			{\bf Return} $\mu < \xi$
		}
	}
\hrule
\end{algorithm}

\begin{theo}\label{thm:behavior-fast-algo}
	Fix a confidence level $\delta > 0$ and an arbitrary reference sequence $\seqn=\{\refseq_i\}_{i=1}^{\infty}$. Suppose that the given instance has a gap $\Delta$.
	Let $\terround$ be the smallest $i$ such that $\refseq_i\le\Delta$.
	With probability at least $1-\delta$,
	\TESTSIGN\ determines whether 
	$\mu > \xi$ or $\mu < \xi$ correctly and uses
	$O((\ln\delta^{-1}+\ln \terround)\refseq_{\terround}^{-2})$ samples in total.
\end{theo}

The proof for the above theorem is somewhat similar to the analysis of the \EXPGAPELIMINATION\ algorithm in \cite{karnin2013almost}
(in fact, simpler since there is only one arm).
The details can be found in the appendix.

Now, let $T(\delta,I) = (\ln \delta^{-1} + \ln \terround) \refseq_{\terround}^{-2}$, in which $I$ is a valid \sign\ instance. It is not hard to see $T(\delta,I)$ here is a reasonable time bound.  Algorithm~\ref{algo:FAST-ALGO-SIGN} is \WEAKCORRECTS{T}, so we can apply Theorem~\ref{theo:TRANSFORM1} to make it \EXPCORRECTS{T}.

\begin{cor}\label{cor:pac-algo}
	For \TESTSIGN\ with the reference sequence $\seqn = \{ \refseq_i \}$. After applying the construction in Theorem~\ref{theo:TRANSFORM1}, we have algorithm $\alg$ for \sign\ such that given confidence level $\delta$, it takes $O((\ln \delta^{-1} + \ln \terround) \refseq_{\terround}^{-2}))$ total samples in expectation, and outputs correctly with probability at least $1-\delta$.
\end{cor}

Finally, we prove Theorem~\ref{thm:FAST-ALGO}.

\begin{proofof}{Theorem~\ref{thm:FAST-ALGO}}
	First, we can easily construct a reference sequence $\{ \refseq_i \}$ such that
	\begin{enumerate}
		\item $0 < \refseq_i < 1$ and $\refseq_{i+1} \le \refseq_i/2$ for all $i$.
		\item $T(\refseq_i) \ge i\cdot \refseq_i^{-2}$ for all $i$
		(this is possible since $\limsup_{\Delta \to +0} T(\Delta)/\Delta^{-2} = +\infty$).
	\end{enumerate}
	Then we apply Corollary~\ref{cor:pac-algo} with reference sequence 
	$\{ \refseq_i \}_{i=1}^{+\infty}$.
	Let the algorithm be $\alg$. For any fixed $\delta$, we can see that
	\[
	\lim_{i \to +\infty} \frac{T_\alg(\refseq_i)}{T(\refseq_i)} \le 
	\lim_{i \to +\infty} \frac{C(\ln \delta^{-1} + \ln i) \refseq_i^{-2}}{i \refseq_i^{-2}} = 0,
	\]
	where $C$ is the constant hidden in the big-O in Corollary~\ref{cor:pac-algo}. 
	This implies that
	$
	\liminf_{\Delta \to +0}  T_\alg(\Delta)/T(\Delta) = 0.
	$
\end{proofof}

\begin{rem}
	If we use the reference sequence $\{ \refseq_i = e^{-i} \}$, then by Corollary~\ref{cor:pac-algo}, the constructed algorithm $\alg$ is \CORRECT\ for \sign, and it takes $O(\Delta^{-2}(\ln\delta^{-1} +  \ln\ln\Delta^{-1}))$ samples in expectation on instance with gap $\Delta$.
\end{rem}


==> lowerbound.tex <==
%!TEX root=bestarm.tex

\newcommand{\powconst}{\gamma}

\section{\sign}
\label{sec:signlowerbound}

In this section, we prove the lower bound for \sign, 
where $\xi \in \R$ is a fixed constant.
For simplicity of exposition, we first assume the distributions of the arms 
are Gaussian distributions with $\sigma = 1$ (but the mean is unknown, of course). %Clearly this is a $1$-sub-Gaussian distribution family.
We will discuss how the assumption can be lifted to obtain lower bounds for other distributions
at the end of the section.

\subsection{Notations}

We first introduce some notations. 
Let $\alg$ denote an algorithm for \sign.
Let $A_\mu$ be an arm with mean $\mu$.
Let $T_{\alg}(\Delta) = \max(T_{\alg}(A_{\xi+\Delta}), T_{\alg}(A_{\xi-\Delta}))$. 
Let 
$$
\lowb(\Delta) = \Delta^{-2} \cdot \ln\ln \Delta^{-1},
$$ 
which is the benchmark we want to compare.
Fix an algorithm $\alg$.
For a random event $\event$, 
$\Pr_{\alg,A_\mu}[\event]$ denotes the probability that $\event$ happens if we run $\alg$ on arm $A_\mu$.
For notational simplicity, when $\alg$ is clear from the context, 
we abbreviate it as $\Pr_\mu[\event]$.
Similarly, we write $\Ex_\mu[X]$ as a short hand notation for $\Ex_{\alg,A_\mu}[X]$. 
Let $\indicator\{\text{expr}\}$ be the indicator function 
which equals 1 when $\text{expr}$ is true and 0 otherwise. 
%\lijie{changed $E$ to $\event$.}

Throughout this section, we assume $0<\delta<0.01$ is a fixed constant.
Recall our goal is to prove Theorem~\ref{thm:DENSITYSIGN-DIST-INFORMAL}.
We need to define nature distribution families for the gap parameter $\Delta$.
First, we define function $\granuf: [0,+\infty) \to \R$
to control the distributions.
\begin{defi}
	We say $\granuf: [0,+\infty) \to \R$ is a {\em granularity function} 
	if $\granuf$ is twice differentiable, strictly increasing,  nonnegative and unbounded.
\end{defi}
Next, we define $\discdistr_N(\granuf)$ ($N\in \N$) to be the following discrete probability distribution of 
the gap parameter $\Delta$:
\footnote{
	We stress that this is not a Bayesian setting since 
	we require the algorithm is $\delta$-correct for every \sign\ instance.
}
$$
\discdistr_N(\granuf) := \text{uniform}\{e^{-\granuf(0)},e^{-\granuf(1)}, \ldots, e^{-\granuf(N)}\}.
$$
We use $e^{-\granuf(i)}$ to make sure the limit is zero.
We remark that a choice other than the exponential function is possible, but as we will see, 
the exponential function is the most natural regime to think about the algorithms and lower bounds. 

Similarly, we define the continuous analogue of $\discdistr_i(\granuf)$ as 
$$
\contdistr_N(\granuf) := e^{-\granuf(x)} \quad \text{where } x\sim \text{uniform} [0, N],
$$

Now, we are ready to define what is the meaning of ``Any algorithm requires $\Omega(F(\Delta))$ samples 
for {\em almost all} instances''.
%For any distribution $\paradistr$ of the gap parameter $\Delta$ and an event $E$, 
%we write $\paradistr(E)$ as a short hand notation for $\Pr_{\Delta\sim \paradistr}[E]$.

\begin{defi}\label{defi:lowerbound-almost-everywhere}
	Let $\{\paradistr_N\}_{N=1}^{+\infty}$ be a sequence of distributions, all supported on $(0,1]$.
	We say that any $\delta$-correct algorithm for \sign\ requires $\Omega(F(\Delta))$ samples for almost all instances with 
	respect to $\{\paradistr_N\}_{N=1}^{+\infty}$ 
	if and only if there exists a universal constant $c>0$ such that for any $\delta$-correct algorithm $\alg$, 
	we have that
	$$
	\lim_{N \to +\infty} \paradistr_N(\{\Delta\mid T_{\alg}(\Delta)<c \cdot F(\Delta) \}) = 0.
	$$
\end{defi}

We briefly discuss the reason why we need an infinite sequence of distributions $\{\Gamma_N\}_{N=1}^{+\infty}$.
In the previous section, we have already seen from Theorem~\ref{thm:FAST-ALGO} that 
there is no instance-wise $\Omega(\lowb(\Delta))$ lower bound. 
So we settle for proving that $\Omega(\lowb(\Delta))$ is a lower bound holds for ``almost all instances'' 
with respect to natural distributions (of $\Delta$) over $(0,1]$
(we would like to call $\Omega(\lowb(\Delta))$ an {\em almost instance-wise lower bound}). 
Suppose $\Delta$ follows a fixed distribution $\paradistr$.
Now, let $a_n = \paradistr([2^{-n},2^{-n+1}))$. Clearly we have $\sum_{n=1}^{+\infty} a_n = 1$. Furthermore, we assume there are infinite many $a_n$ such that $a_n > 0$ as otherwise $F(\Delta)$ is bounded by a constant on all instance. 
Fix $n$ and consider the algorithm $\alg_n$, which is obtained by applying
Corollary~\ref{cor:pac-algo} with the reference sequence $\{ \refseq_i = 2^{-n+1-i} \}_{i=1}^{+\infty}$. 
We can see the algorithm uses less than $O(\Delta^{-2}) = o(\lowb(\Delta))$ number of samples in expectation   
if $\Delta\in [2^{-n},2^{-n+1})$. It means for any $c>0$, we can pick a big enough $n$ with $a_n > 0$ such that $\paradistr(\{ \Delta\betw T_{\alg_n}(\Delta) < c \cdot \lowb(\Delta) \}) \ge a_n > 0$.
However, the existence of such $\alg_n$ which can solve a nontrivial proportion of instances faster
is not a very useful or insightful result as we do not know $n$ and $\alg_n$ (for large $n$) 
clearly is not a very good algorithm. 
To resolve this issue, we use an infinite sequence of distributions  $\{\paradistr_N\}_{N=1}^{+\infty}$,
instead of a single distribution,
and investigate the limiting behavior of any algorithm.

If the granularity function $\granuf$ behaves arbitrarily, it seems to be impossible to analyze the problem. 
However, for $\granuf$ being either convex or concave, we manage to provide complete 
characterization when \sign\ requires $\Omega(F(\Delta))$ for almost all instances.
The main results of this section are the following theorems.

\begin{theo} 
	\label{thm:DENSITYSIGN-DIST-CONVEX}
	(Almost instance-wise lower bound, for convex granularity function)
	Let $\granuf$ be a convex granularity function.
	Any $\delta$-correct algorithm for \sign\ needs $\Omega(\lowb(\Delta))$ samples 
	for almost all instances with respect to $\{\discdistr_N(\granuf) \}_{N=1}^{+\infty}$ 
	iff there exists $\powconst>0$ such that $\granuf(x)=O(x^\powconst)$. 
	
	In other words, the lower bound holds iff $\granuf(x)$ grows no faster than some polynomial function.
	
	For the continuous case, any $\delta$-correct algorithm for \sign\ requires $\Omega(\lowb(\Delta))$ samples 
	for almost all instances with respect to $\{\contdistr_N(\granuf) \}_{N=1}^{+\infty}$. 
\end{theo}

%\lijie{Corrected the above theorem, as the lower bound holds for all convex function in the continuous case. Maybe we need some words to explain why continuous and discrete versions are different.}

It may seem strange that the result for the discrete case differs from that for the continuous analogue
for convex granularity functions. 
Intuitively, the reason is as follows:
if $\granuf(x)$ grows faster than any polynomial, then we can design a reference sequence 
to make all the points $e^{\granuf(i)}, i\in \mathbb{N}$ fast points.
However, in the continuous case, the span of each interval $[e^{\granuf(i+1)}, e^{\granuf(i)})$
is too large in some sense, 
and being quick at its endpoints does not make the whole interval quick points.
But for concave granularity functions, such difference does not exist, as 
in the following theorem.

\begin{theo} 
	\label{thm:DENSITYSIGN-DIST-CONCAVE}
	(Almost instance-wise lower bound, for concave granularity function)
	Let $\granuf$ be a concave granularity function.
	Any $\delta$-correct algorithm for \sign\ needs $\Omega(\lowb(\Delta))$ samples
	for almost all instances with respect to $\{\discdistr_N(\granuf) \}_{N=1}^{+\infty}$ 
	iff there exists $\powconst>0$ such that $\liminf_{x \to +\infty} \frac{x\granuf'(x)}{\granuf(x)^\powconst} > 0$.
	The same statement holds for $\{\contdistr_N(\granuf) \}_{N=1}^{+\infty}$ as well.
\end{theo}

\eat{
\lijie{The previous statements is somehow inaccurate, the previous statements means for any $\delta$-correct algorithm $\alg$ , there exists $c_1$ such that it need $c_1\cdot \lowb$ samples almost everywhere, but indeed our results is that there exists $c_1$ such that for any $\delta$-correct algorithm $\alg$ it requires $c_1 \cdot \lowb$ samples everywhere. It is not the same. I correct it, maybe now you should change the informal statement in the introduction a little bit too.}
}

The rest of the section is devoted to prove the above two theorems.
We need a few notations.
For an integer $N \in \mathbb{N}$,
a $\delta$-correct algorithm $\alg$ for \sign,
and a function $g : \R \to \R$, 
define
$$
\distportion(\alg,g,N) = \sum_{i=1}^{N} \indicator\left\{ \text{There exists some } \Delta \in [e^{-i},e^{-i+1}) \text{ such that: } T_{\alg}(\Delta) < g(\Delta) \right\}.
$$ 
Intuitively, it is the number of intervals $[e^{-i},e^{-i+1})$ among the first $N$ intervals that contains a fast point with respect to $g$.

The following two lemmas are crucial to us, and may be useful for proving lower bounds for related problems.


\begin{lemma}\label{lm:FRACTION-BOUND-DISC}
	For any $\powconst>0$, we have a constant $c_1>0$ (which depends on $\powconst$) such that
	\[
	\lim_{N \to +\infty} \sup_{\alg' \text{ is } \delta\text{-correct} } \frac{\distportion(\alg',c_1 \lowb, N)}{N^\powconst} = 0.
	\]
	%	In which $c_1\lowb$ is interpreted as the function $(c_1\lowb)(x) = c_1 \cdot \lowb(x)$.
	In other words, the number of intervals containing fast points with respect to $\Omega(\lowb)$ can be smaller than any polynomial. 
\end{lemma}

\noindent
Lemma~\ref{lm:FRACTION-BOUND-DISC} has a continuous analogue.
For $N \in \mathbb{N}$ and function $g : \R \to \R$, 
let 
$$
\contportion(\alg,g,N) = \int_{0}^{N} \indicator\left\{T_{\alg}(e^{-x}) < g(e^{-x})\right\} \d x.
$$
That is the mass of fast points with respect to $g$ in interval $[0,N]$.

\begin{lemma}\label{lm:FRACTION-BOUND-CONTINUOUS}
	For any $\powconst>0$, we have a constant $c_1>0$ (which depends on $\powconst$) such that
	\[
	\lim_{N \to +\infty} \sup_{\alg' \text{ is } \delta\text{-correct} } \frac{\contportion(\alg',c_1 \lowb,N)}{N^\powconst} = 0.
	\]
	In other words, the mass of fast points with respect to $\Omega(\lowb)$ can be smaller than any polynomial. 
\end{lemma}

The proofs of Theorem~\ref{thm:DENSITYSIGN-DIST-CONVEX} and Theorem~\ref{thm:DENSITYSIGN-DIST-CONCAVE} 
are largely based on
Lemma~\ref{lm:FRACTION-BOUND-DISC}, Lemma~\ref{lm:FRACTION-BOUND-CONTINUOUS} and Corollary~\ref{cor:pac-algo}
and the properties of convex/concave functions.
The ideas of the proofs are not difficult, but the details of the calculations are somewhat tedious, which 
we defer to the appendix. 
Below we provide the proofs for Lemma~\ref{lm:FRACTION-BOUND-DISC} and Lemma~\ref{lm:FRACTION-BOUND-CONTINUOUS}, 
which contain the core ideas of our lower bound. 

\eat{
	\topic{Organization of the proofs}
	
	Since the proof contains several parts, we briefly outline the organization of the proofs. We first prove Lemma~\ref{lm:FRACTION-BOUND-DISC}, which is most challenging. In order to prove it, we introduce a new novel idea besides the original change of distribution. Then Lemma~\ref{lm:FRACTION-BOUND-CONTINUOUS} is a simple consequence of Lemma~\ref{lm:FRACTION-BOUND-DISC}.
	
	Then we prove Theorem~\ref{thm:DENSITYSIGN-DIST-CONVEX} and Theorem~\ref{thm:DENSITYSIGN-DIST-CONCAVE}. They all contain two parts, one states that if granularity function $\granuf$ meets certain criterion, then the lower bound holds, another one states that if it doesn't meet that criterion, then there exists a fast algorithm. For the first part, we carefully apply Lemma~\ref{lm:FRACTION-BOUND-DISC} or Lemma~\ref{lm:FRACTION-BOUND-CONTINUOUS}. And for the second part, we build the desired algorithm by using the framework introduced in Section~\ref{sec:algorithm-sign}.
}

\subsection{Proof for Lemma~\ref{lm:FRACTION-BOUND-DISC} and Lemma~\ref{lm:FRACTION-BOUND-CONTINUOUS}}

We first show a simple but convenient lemma based on Lemma~\ref{lm:CHANGEDIST}.

%\lijie{The above event should also be an ending event.}
\begin{lemma}\label{lm:BIGHURTSMALL}
	Let $I_1$ (with reward distribution $\distr_1$) and $I_2$ (with reward distribution $\distr_2$)
	be two instances of \sign.  
	Let $\event$ be a random event and 
	$\tau$ be the total number of samples taken by $\alg$.
	Suppose $\Pr_{\distr_1}[\event] \ge \frac{1}{2}$.
	Then, we have	
	\[
	\Pr_{\distr_2}[\event] \ge \frac{1}{4}\exp\bigl(-2\Ex_{\distr_1}[\tau]\KL(\distr_1,\distr_2)\bigr).
	\]
\end{lemma}

\begin{proof}
	Applying Lemma~\ref{lm:CHANGEDIST}, we have that
	\[
	\Ex_{\distr_1}[\tau] \cdot \KL(\distr_1,\distr_2) \ge \ent(\Pr_{\distr_1}[\event],\Pr_{\distr_2}[\event]) 
	\ge 
	\ent\left(\frac{1}{2},\Pr_{\distr_2}[\event]\right) 
	\ge \frac{1}{2} \cdot \ln\left(\frac{1}{4\Pr_{\distr_2}[\event](1-\Pr_{\distr_2}[\event])}\right).
	\]
	Hence, we can see that 
	$
	4\Pr_{\distr_2}[\event](1-\Pr_{\distr_2}[\event]) \ge \exp(-2\Ex_{\distr_1}[\tau]\cdot \KL(\distr_1,\distr_2)),
	$
	from which the lemma follows easily.
\end{proof}

From now on, suppose $\alg$ is a $\delta$-correct algorithm for \sign.
We define two events:
$$
\event_U = [\alg \text{ outputs }``\mu>\xi"],
$$
$$
\event(\Delta) = \event_U \wedge [ d\Delta^{-2} \le \tau \le 5 T_{\alg}(\Delta) ],
$$
where 
$\tau$ is the number of samples taken by $\alg$ and
$d$ is a universal constant to be specified later. The following lemma is a key tool, which can be used to partition the event $\event_U$ into several disjoint parts. 

\begin{lemma}
	\label{lm:EVENTEXT}
	For any $\Delta > 0$ and $d < \ent(0.2,0.01)/2$, we have that
	$$
	\Pr_{\xi+\Delta}[\event(\Delta)]=\Pr_{\alg, A_{\xi+\Delta}}[\event(\Delta)] \ge \frac{1}{2}.$$
\end{lemma} 

\begin{proof} 	
	First, we can see that $\Pr_{\xi+\Delta}[\event_U] \ge 1-\delta \ge 0.99$
	since $\alg$ is $\delta$-correct and ``$\mu>\xi$" is the right answer.
	
	Now, we claim $\Pr_{\xi+\Delta}[\tau < d\Delta^{-2}] < 0.25$.
	Suppose to the contrary that
	$\Pr_{\xi+\Delta}[\tau < d\Delta^{-2}] \ge 0.25$. 
	We can see that $\Pr_{\xi+\Delta}[\event_U \wedge \tau < d\Delta^{-2}] \ge 0.25 - \delta  > 0.2$.
	
	Consider the following algorithm $\alg'$:
	$\alg'$ simulates $\alg$ for $d \Delta^{-2}$ steps. 
	If $\alg$ halts, $\alg'$ outputs what $\alg$ outputs, 
	otherwise $\alg'$ outputs nothing. 
	
	Let $\event_V$ be the event that $\alg'$ outputs $\mu > \xi$.
	Clearly, we have $\Pr_{\alg',\xi+\Delta}[\event_V] > 0.2$. 
	On the other hand, $\Pr_{\alg',\xi-\Delta}[\event_V] < \delta$,
	since $\alg$ is a $\delta$-correct algorithm. 
	So by Lemma~\ref{lm:CHANGEDIST}, we have that
	\[
	\Ex_{\alg',\xi+\Delta}[\tau] \KL(N(\xi+\Delta,\sigma),N(\xi-\Delta,\sigma)) = 
	\Ex_{A',\xi+\Delta}[\tau] 2\Delta^{2} \ge \ent(0.2,\delta) \ge \ent(0.2,0.01).
	\]
	
	
	Since $d \Delta^{-2} \ge \Ex_{\alg',\xi+\Delta}[\tau]$, we have $d \ge \ent(0.2,0.01)/2$.
	But this contradicts the condition of the lemma. 
	Hence, we must have $\Pr_{\xi+\Delta}[\tau < d\Delta^{-2}] < 0.25$.
	
	Finally, we can see that
	\begin{align*}
	\Pr_{\xi+\Delta}[\event(\Delta)] &\ge \Pr_{\xi+\Delta}[\event_U] - \Pr_{\xi+\Delta}[\tau < d\Delta^{-2}] - \Pr_{\xi+\Delta}[\tau > 5 T_\alg(\Delta)] \\
	&\ge 1-0.01-0.25 - \Pr_{\xi+\Delta}[\tau > 5 \Ex_{\alg,\xi+\Delta}[\tau]]\\
	&\ge 1-0.01-0.25-0.2 \ge 0.5
	\end{align*}
	where the first inequality follows from the union bound and the second from Markov inequality.
\end{proof}

%\lijie{change the below to be the finite sum, as we only make use of this.}

\begin{lemma}
	\label{lm:sequence-bound}
	For any $\delta$-correct algorithm $\alg$, and any finite sequence $\{\Delta_i\}_{i=1}^{n}$ 
	such that 
	\begin{enumerate}
		\item the events $\{\event(\Delta_i)\}$ are disjoint, 
		\footnote{
			More concretely, the intervals $[d\Delta_i^{-2}, 5T_{\alg}(\Delta_i)]$ are disjoint.
		}
		and $0 < \Delta_{i+1} < \Delta_i$ for all $1 \le i \le n-1$;
		\item there exists a constant $c>0$ such that $T_{\alg}(\Delta_i)\leq c \cdot \lowb(\Delta_i) $ for all $1\le i \le n$,
	\end{enumerate}
	then it must hold that:
	\[
	\sum_{i=1}^{n} \exp\{-2c\cdot \lowb(\Delta_i)\cdot \Delta_i^2\} \le 4\delta.
	\]
\end{lemma}

\begin{proof}	
	Suppose for contradiction that 
	$\sum_{i=1}^{n} \exp\{-2c\cdot \lowb(\Delta_i)\cdot \Delta_i^2\} 
	> 4 \delta$.
	
	Let $\alpha = \frac{1}{5}\Delta_n$. 
	By Lemma~\ref{lm:NORMALKL}, 
	we can see that $\KL(\Normal(\xi+\Delta_i,\sigma),\Normal(\xi-\alpha,\sigma)) 
	= \frac{1}{2\sigma^2} (\Delta_i+\alpha)^2 \le \frac{1}{2}(1.2\Delta_i)^2 \le  \Delta_i^2$.
	By Lemma~\ref{lm:BIGHURTSMALL}, we have:
	\[
	\Pr_{\xi-\alpha}[\event_U] \ge \sum_{i=1}^{n} \Pr_{\xi-\alpha}[\event(\Delta_i)] 
	\ge \frac{1}{4} \sum_{i=1}^{n} \exp\{-2 \Ex_{\xi+\Delta_i}[\tau]\, \Delta_i^2\}
	\ge \frac{1}{4} \sum_{i=1}^{n} \exp\{-2 c\cdot \lowb(\Delta_i)\cdot \Delta_i^2\}>\delta.
	\]
	Note that we need Lemma~\ref{lm:EVENTEXT}(1) (i.e., $\Pr_{\xi+\Delta_i}[\event(\Delta_i)]\geq 1/2$ ) 
	in order to apply Lemma~\ref{lm:BIGHURTSMALL} for the second inequality.
	The above inequality means that    
	$\alg$ outputs a wrong answer for instance $\xi-\alpha$ with probability $>\delta$,
	which contradicts that $\alg$ is $\delta$-correct.
\end{proof} 

%TODO: reorganize below a bit.

%	With the help of Lemma~\ref{lm:converging}, the rest of the proof of Theorem~\ref{thm:DENSITYSIGN}
%	goes as follows:
%	Suppose the $\lim\sup$ in Theorem~\ref{thm:DENSITYSIGN} is not zero, but some positive constant,
%	for some $\delta$-correct algorithm algorithm $\alg$. 
%	So there is a positive constant fraction of $\Delta$ values such that $T_\alg(\Delta)<\granuf(\Delta)$.
%	We show that we can extract a sequence $\Delta_1, \Delta_2, \ldots$ such that 
%	(1) $\{\event(\Delta_i)\}_i$ are disjoint, (2)  $T_\alg(\Delta_i)<\granuf(\Delta_i)$ for all $i$,
%    but (3) $\sum_{i=1}^{+\infty} \exp\{-4\cdot \granuf(\Delta_i)\cdot \Delta_i^2\} > 4\delta$.
%    This renders a contradiction to Lemma~\ref{lm:converging}.

Now, we try to utilize Lemma~\ref{lm:sequence-bound} on a carefully constructed sequence $\{\Delta_i\}$.
The construction of the sequence $\{\Delta_i\}$ requires quite a bit calculation.
To facilitate the calculation, we provide a sufficient condition for the disjointness of the sequence, as follows.

\begin{lemma}\label{lm:DISJOINT-EVENTS}
	$\alg$ is any $\delta$-correct algorithm for \sign.
	$c>0$ is a universal constant.
	The sequence $\{\Delta_i\}_{i=0}^N$ satisfies the following properties: 
	\begin{enumerate}
		\item $1/e>\Delta_1>\Delta_2>\dotsc>\Delta_N\ge\alpha>0$.
		\item For all $i\in [N]$, we have that $T_{\alg}(\Delta_i) \le c\cdot \lowb(\Delta_i)$.
		\item Let $L_i = \ln \Delta_i^{-1}$.
		We have $L_{i+1} - L_{i} > \frac{1}{2}\ln\ln\ln\alpha^{-1} + c_1$, in which $c_1 = \frac{\ln c + \ln 5 - \ln d}{2}$.
	\end{enumerate}
	Then, the events $\{\event(\Delta_1), \event(\Delta_2), \ldots, \event(\Delta_N)\}$  are disjoint. 
\end{lemma}

\begin{proof}
	We only need to show the intervals for each $\event(\Delta_i)$ are disjoint. 
	In fact, it suffices to show it holds for two adjacent events $\event(\Delta_i)$ and $\event(\Delta_{i+1})$. 
	Since $5T_{\alg}(\Delta_i) \le 5c\cdot\lowb(\Delta_i)$, we only need to show	
	$
	5c\cdot\lowb(\Delta_i) < d \Delta_{i+1}^{-2},
	$
	which is equivalent to
	\[
	\ln c + \ln 5 + 2 L_{i} + \ln\ln L_{i} < \ln d + 2 L_{i+1}.
	\]
	By simple manipulation, this is further equivalent to 
	$L_{i+1} - L_{i} > (\ln c + \ln 5 - \ln d + \ln\ln L_{i})/2$.	
	Since $\alpha \le \Delta_i$, we have $\ln\ln\ln \alpha^{-1} \ge \ln\ln L_i$, which concludes the proof. 
\end{proof}

Now, everything is ready to prove Lemma~\ref{lm:FRACTION-BOUND-DISC}.

\begin{proofof}{Lemma~\ref{lm:FRACTION-BOUND-DISC}}
	Suppose for contradiction, for any $c_1 > 0$, the limit is not zero.
	This is equivalent to
	\begin{align}
	\label{eq:limsup1}
	\limsup_{N \to +\infty} \sup_{\alg' \text{ is } \delta-\text{correct} } \frac{\distportion(\alg',c_1 \lowb, N)}{N^\powconst} > 0.
	\end{align}
	We claim that for $c_1 = \frac{\powconst}{4}$, the above can lead to a contradiction.
	
	%	Suppose
	
	%	\[
	%	\limsup_{N \to +\infty} \sup_{\alg' \text{ is } \delta-\text{correct} } \frac{C(\alg',c_1 \lowb, N)}{N^c} = 2\alpha > 0.
	%	\]
	
	First, we can see that \eqref{eq:limsup1} is equivalent to 
	the existence of an infinite increasing sequence $\{N_i\}_i$ and a positive number $\beta>0$
	such that
	\[
	\sup_{\alg' \text{ is } \delta-\text{correct} } \frac{\distportion(\alg',c_1 \lowb, N_i)}{N_i^\powconst} > \beta, \quad \text{ for all }i.
	\]
	
	Consider some large enough $N_i$ in the above sequence.
	The above formula implies that there exists a $\delta$-correct algorithm $\alg$ 
	such that $\distportion(\alg,c_1\lowb, N_i) \ge \beta N_i^{\powconst}$.
	
	We maintain a set $S$, which is initially empty.
	For each $2\le j\le N_i$, if there exists $\Delta \in [e^{-j},e^{-j+1})$ such that
	$T_{\alg}(\Delta) \le c_1 F(\Delta)$, 
	then we add one such $\Delta$ into the set $S$. 
	We have $|S| \ge \distportion(\alg,c_1\lowb,N_i) -1 \ge \beta N_i^\powconst - 1$
	($-1$ comes from that $j$ starts from 2).
	Let 
	$$
	b = \left\lceil \frac{\ln c_1 + \ln 5 - \ln d +\ln\ln N_i}{2} + 1 \right\rceil.
	$$ 
	We keep only the $1$st, $(1+b)$th, $(1+2b)$th, $\dotsc$ elements in $S$, and remove the rest.
	With a slight abuse of notation, rename the elements in $S$ by
	$\{ \Delta_{i} \}_{i=1}^{|S|}$, sorted in decreasing order. 
	
	It is not difficult to see that $\frac{1}{e}>\Delta_1 >\Delta_2>\dotsc>\Delta_{|S|} \ge e^{-N_i}>0$.
	By the way we choose the elements, for $1 \le i < |S|$, 
	we have 
	$$
	\ln \Delta_{i+1}^{-1} - \ln\Delta_{i}^{-1} > \frac{\ln c_1 + \ln 5 - \ln d}{2} +  \frac{1}{2}\ln\ln N.
	$$ 
	Recall that we also have $T_{\alg}(\Delta_i) \le c_1 \lowb(\Delta_i)$ for all $i$. 
	Hence, we can apply Lemma~\ref{lm:DISJOINT-EVENTS} and conclude that all events $\{\event(\Delta_i)\}$ are disjoint.
	
	We have $|S|\ge (\beta N_i^\powconst-1)/b$, for large enough $N_i$ (we can choose such $N_i$ since $\{N_i\}$ approaches to
	infinity), it implies $|S| \ge \beta N_i^\powconst/\ln\ln N_i$. Then, we can get
	\begin{align*}
	\sum_{j=1}^{|S|} \exp\{-2c_1\cdot \lowb(\Delta_j)\cdot\Delta_j^{-2}\} 
	=&\sum_{j=1}^{|S|} \exp\{-\powconst\cdot \ln\ln \Delta_j^{-1}/2\}\\
	=&\sum_{j=1}^{|S|} (\ln \Delta_j^{-1})^{-\powconst/2}
	\ge |S| \cdot N_i^{-\powconst/2}\\
	\ge& \beta N_i^\powconst/\ln\ln N_i \cdot N_i^{-\powconst/2} = \beta N_i^{\powconst/2}/\ln\ln N_i.
	\end{align*}
	The inequality in the second line holds since $\Delta_j\geq e^{-N_i}$ for all $j\in [|S|]$.
	Since $\powconst>0$, we can choose $N_i$ large enough such that $\beta N_i^{\powconst/2}/\ln\ln N_i > 4\delta$, which renders a contradiction to Lemma~\ref{lm:sequence-bound}.
\end{proofof}

Now we prove Lemma~\ref{lm:FRACTION-BOUND-CONTINUOUS}, which is a simple consequence of Lemma~\ref{lm:FRACTION-BOUND-DISC}.

\begin{proofof}{Lemma~\ref{lm:FRACTION-BOUND-CONTINUOUS}}
	The lemma follows from the following observation:
	%	For any $\delta$-correct algorithm $\alg$, function $g : \R \to \R$ 
	\begin{align*}
	\contportion(\alg,g,N) &\le \int_{0}^{\lceil N \rceil} \indicator\{ T_{\alg}(e^{-x}) < g(e^{-x}) \} dx \\
	&= \sum_{i=1}^{\lceil N \rceil} \int_{i-1}^{i} \indicator\{ T_{\alg}(e^{-x}) < g(e^{-x}) \} dx\\
	&\le \sum_{i=1}^{\lceil N \rceil} \indicator\{ \text{There exists } \Delta \in [e^{-i},e^{-i+1}) \text{ such that: } T_{\alg}(\Delta) < g(\Delta) \}\\
	&\le \distportion(\alg,g,\lceil N \rceil).
	\end{align*}
	Hence this lemma just follows from Lemma~\ref{lm:FRACTION-BOUND-DISC}.
\end{proofof}

\subsection{Generalization to other distributions}
\label{subsec:generalization}

In this subsection, we briefly discuss how to generalize our results to other 1-sub-Gaussian distributions as well.
Note that all our proofs rely on Corollary~\ref{cor:pac-algo} (for the upper bound) and Lemma~\ref{lm:FRACTION-BOUND-DISC}
(for the lower bound). It is easy to see that 
Corollary~\ref{cor:pac-algo} works for all 1-sub-Gaussian distributions. 
For Lemma~\ref{lm:FRACTION-BOUND-DISC}, the only property of the distributions we used is 
the KL divergence through Lemma~\ref{lm:CHANGEDIST}. 
Hence, we can use our framework to handle other classes of distributions with similar mean-KL-divergence relations.
%Intuitively Speaking, this technique relies on the fact that the distributions of two arm with close mean are also close in a certain sense, so the algorithm must make efforts to distinguish them. 
More concretely, let $\mathcal{M}$ be a specific class of reward distributions (all having 1-sub-Gaussian tail).
%\footnote{By the assumption of the problem, they all .}, 
Each distribution in $\mathcal{M}$ is uniquely indexed by its mean. 
Let $\distr_\mu \in \mathcal{M}$ denote the distribution with mean $\mu$. We also assume all the means lie in range $(a,b)$.  
For each $\mu \in (a,b)$, there exists a corresponding reward distribution $\distr_\mu \in \mathcal{M}$. 
Suppose for all $\mu_1,\mu_2 \in (a,b)$, we have $\KL(\distr_{\mu_1},\distr_{\mu_2}) \le C |\mu_1 - \mu_2|^2$ for some constant $C > 0$. 
Then, all our previous proofs work exactly in the same way and Theorem~\ref{thm:DENSITYSIGN-DIST-CONVEX} and Theorem~\ref{thm:DENSITYSIGN-DIST-CONCAVE} 
also hold for any $\delta$-correct algorithm $\alg$ for \sign.

As an important example, the class of Bernoulli distributions exhibits the above property. Let $\mathcal{B}_\mu$ denote the Bernoulli distribution with mean $\mu$. We have $\KL(\mathcal{B}_{p},\mathcal{B}_q) \le \frac{(p-q)^2}{q(1-q)}$ (see (2.8) in \cite{bubeck2012regret}). 
Then for all $0<\epsilon<0.5$, for all $p,q \in (0.5-\epsilon,0.5+\epsilon)$, we have that
\[
\KL(\mathcal{B}_{p},\mathcal{B}_{q}) \le \frac{4}{1-4\epsilon^{2}} |p-q|^2,
\]
since $q(1-q) \ge (0.5-\epsilon)(0.5+\epsilon)$ for $q\in(0.5-\epsilon,0.5+\epsilon)$.

This shows for any $0 < \epsilon <0.5$ and $\xi \in (0.5-\epsilon,0.5+\epsilon)$, Theorem~\ref{thm:DENSITYSIGN-DIST-CONVEX} and Theorem~\ref{thm:DENSITYSIGN-DIST-CONCAVE} hold for all $\delta$-correct algorithms for \sign\ when all reward distributions are Bernoulli.


==> upperbound.tex <==
%!TEX root=bestarm.tex

\section{Lower Bound for BEST-1-ARM}
	
	\begin{theo}(Density of good fraction for \textbf{bestarm} is 0)\label{DENSITYBESTARM}
		There is a universal constant $c$ such that:
		
		For any fixed $\mu_1$.
		
		Let $f(\mu_1,\dotsc,\mu_n) = c \cdot \sum_{i=2}^{n} \Delta_i^{-2} \ln\ln \Delta_i^{-1}$.(Recall that $\Delta_i =\mu_i - \mu_1$.)
		Let $g(A,x_2,\dotsc,x_n) = [T_{A}(\mu_1,\mu_1-e^{-x_2},\mu_1-e^{-x_3},\dotsc,\mu_1-e^{-x_n}) < f(\mu_1,\mu_1-e^{-x_1},\mu_1-e^{-x_2},\dotsc,\mu_1-e^{-x_n})]$
		
		Given $N$, let $\tau_N$ be:
		
		\[
		\sup_{C\text{ is a }\delta\text{-PAC for \textbf{bestarm}}} \frac{1}{N^{n-1}} \cdot \int_{0}^{N}\dotsc \int_{0}^{N} g(C,x_2,x_3,\dotsc,x_n) d\mathbf{x}.\footnote{$d\mathbf{x}$ means $ dx_2dx_3\dotsc dx_{n}$}
		\]
		
		Then we have:
		\[
		\lim_{N \to +\infty} \tau_N = 0.
		\]
		
		for any $\delta < 0.01$.
	\end{theo}
	
	\begin{cor}		
		Let $A$ be a $\delta$-PAC for \textbf{bestarm}, for $\delta < 0.01$, there is a universal constant $c$ such that:
		
		For any fixed $\mu_1$, let $f,g$ denote the same functions as in Lemma~\ref{DENSITYBESTARM}.
		
		\[
		\limsup_{N \to + \infty}  \frac{1}{N^{n-1}} \cdot \int_{0}^{N}\dotsc \int_{0}^{N} g(A,x_2,x_3,\dotsc,x_n) d\mathbf{x}= 0.
		\]
		
		That is, on the logarithm granularity, the density for "quick points" approaches to 0.
	\end{cor}
	
	\begin{proof}
		By the definition of $\tau_{N}$, for all $N$, we have:
		\[
		\frac{1}{N^{n-1}} \cdot \int_{0}^{N}\dotsc \int_{0}^{N} g(A,x_2,x_3,\dotsc,x_n) d\mathbf{x} \le \tau_N
		\]
		
		Thus:
		
		\[
	\limsup_{N \to + \infty}  \frac{1}{N^{n-1}} \cdot \int_{0}^{N}\dotsc \int_{0}^{N} g(A,x_2,x_3,\dotsc,x_n) d\mathbf{x}
		\le \limsup_{N \to + \infty} \tau_N = 0.
		\]
	\end{proof}
	
	Now we turn to prove Theorem~\ref{DENSITYBESTARM}, we will reduce it to the case of Theorem~\ref{DENSITYSIGN}.
	
	\begin{proof}
		
	We set $c=\frac{1}{8}$ as in the proof of Theorem~\ref{DENSITYSIGN}.	
		
	Suppose not, then we have:
	
	\[
	\limsup_{N \to +\infty} \tau_N = \alpha > 0.
	\]
	
	Which means there exists a sequence $\{N_i\}$ s.t. $\lim_{i \to +\infty} N_i = +\infty$ and for every $i$, $\tau_{N_i} > \frac{3}{4}\alpha$.
	
	Now, suppose $\tau_{N} > \frac{3}{4}\alpha$. Then, by the definition of $\tau_{N}$, there exists a $\delta$-PAC $C_N$ for \textbf{bestarm} s.t. 
	
	\[
	\frac{1}{N^{n-1}} \cdot \int_{0}^{N}\dotsc \int_{0}^{N}
	g(C_N,x_2,x_3,\dotsc,x_n)d\mathbf{x} > \frac{\alpha}{2}.
	\]
	
	Now, let 
	\[
	g_{i}(C,x_2,x_3,\dotsc,x_n) = [\Ex_{C,v}[\tau_i] < c\Delta_i^{-2} \ln\ln \Delta_i^{-1}]
	\]
	
	In which $v=(\mu_1,\mu_1-e^{-x_2},\dotsc,\mu_1-e^{-x_n})$.
	
	Note that, if $g(C,x_2,x_3,\dotsc,x_n) = 1$, then $\sum_{i=2}^{n} \Ex_{C,v}[\tau_i] \le \Ex_{C,v}[\tau] < \sum_{i=2}^{n} c\Delta_i^{-2} \ln\ln \Delta_i^{-1}$. Clearly, this means there must exists $2 \le i \le n$ s.t. $\Ex_{C,v}[\tau_i] < c\Delta_i^{-2} \ln\ln \Delta_i^{-1}$. Thus we have:
	
	\[
	g(C,x_2,x_3,\dotsc,x_n) \le \sum_{i=2}^{n} g_i(C,x_2,x_3,\dotsc,x_n).
	\]
	
	So we have:
	\[
	\frac{1}{N^{n-1}} \cdot \int_{0}^{N}\dotsc \int_{0}^{N}
	\sum_{i=2}^{n} g_i(C_N,x_2,x_3,\dotsc,x_n)d\mathbf{x} > \frac{\alpha}{2}
	\]
	
	Which means that there exists $i$ s.t.
	
	\[
	\frac{1}{N^{n-1}} \cdot \int_{0}^{N}\dotsc \int_{0}^{N}
	\sum_{i=2}^{n} g_i(C_N,x_2,x_3,\dotsc,x_n)d\mathbf{x} > \frac{\alpha}{2(n-1)}.
	\]
	
	WOLG assume $i=2$, then clearly there must exists $y_3,y_4,\dotsc,y_n \in [0,N]$ s.t.
	
	\[
	\int_{x_2=0}^{N} g_{i}(x_2,y_3,y_4,\dotsc,y_n) dx_2 > \frac{\alpha}{2(n-1)} \cdot N.
	\]
	
	Now, consider the following two algorithms $A_N$ for $\textbf{sign}_{\mu_1}$.
	
	$A_N$:
	\begin{itemize}
	\item Given an arm with payoff distribution $N(\mu,\sigma)$, with unknown $\mu$.
	\item Set $\mu_i = \mu_1 - e^{-y_i}$ for $i>2$.
	\item Simulate $C_N$, whenever $C_N$ ask to pull from arm $i \ne 2$, simulate it with $N(\mu_i,\sigma)$.
	\item Otherwise, pull the arm $N(\mu,\sigma)$.
	\item When $C_N$ terminates, let $\hat{i}$ denote its output, return $\mu > \mu_1$ if $\hat{i}=2$, otherwise return $\mu < \mu_1$.
	\end{itemize}
	
	Since $C_N$ is a $\delta$-PAC for \textbf{bestarm}, it is easy to see $A_N$ is a $\delta$-PAC for $\textbf{sign}_{\mu_1}$.
	
	Let $x_2 \in [0,N]$, and $\Delta = e^{-x_2}$. Then we can see on input $N(\mu_1-\Delta,\sigma)$, the running time for $A_N$ is just $\Ex_{C_N,v}[\tau_2]$, 
	in which $v=(\mu_1,\mu_1-e^{-x_2},\dotsc,\mu_1-e^{-x_n})$.
	
	But we have:
	\[
	\int_{x_2=0}^{N} g_{i}(x_2,y_3,y_4,\dotsc,y_n) dx_2 > \frac{\alpha}{2(n-1)} \cdot N.
	\]
	
	Which means:
	\[
	\int_{x=0}^{N} [T_{A_N}(-e^{-x}) < c \Delta_i^{-2} \ln\ln \Delta_i^{-1}] dx > \frac{\alpha}{2(n-1)} \cdot N.
	\]
	
	But this means that for all $\{N_i\}$, we have $\gamma_{N_i} > \frac{\alpha}{2(n-1)} \cdot N$. by Remark~\ref{SYMREMARK},  This contradicts Theorem~\ref{DENSITYSIGN}
	
\end{proof}

